Glueballs in Flatland

The pure gauge theory in 2+1 dimensions is explored, through both a phenomenological model and a lattice calculation. The Isgur-Paton model is extended to include a curvature term and various mixing mechanisms. The method of inferential statistics is used to extract the parameters of best fit and to compare the likelihoods of the various models when compared to existing lattice data. The conventional assignment of spin 0 to the pseudoscalar state is called into question by the proximity of a spin 4 state in the model, which motivates calculating the mass of the spin 4 state on the lattice. Novel lattice operators are constructed from a matrix of effective Greens functions which attempt to overcome the lattice rotational ambiguities. Correlation functions are presented for the channels with even J, and effective masses extracted. The resulting masses compare well with the extended Isgur-Paton model.

==> intro.tex <==
\chapter{Introduction} \label{chap:intro}

\section{The first section} \label{sect:thefirst}

What the hell is a glueball?  How the fuck should I know?  Everyone
always waves their hands and yells ``nonperturbative effects'' while
those math geeks that like to push pencils draw crazy little diagrams
and argue over integrals without actually thinking up a damn thing.
Glueballs are round, more or less, and vibrating.  Sounds kinky, don't
it?  Well, having glueballs is certainly not a good state to be in,
now is it?

==> latreview.tex <==
\chapter{Details of the Lattice Calculation} \label{chap:latreview}



